IBLTs Measure Before They Decode: Self-Sizing Set Reconciliation for Database Consistency Verification

Cross-system data replication pipelines cannot confirm end-to-end consistency from the local guarantees of each hop, so the two endpoints must be compared directly on a periodic basis. Once the rows of a fixed snapshot are normalized into fingerprints, the task reduces to finding the symmetric difference of the two sets. An Invertible Bloom Lookup Table (IBLT) reconciles the sets with communication that grows only with the difference cardinality $d$, independent of table size, but its capacity must be fixed while $d$ is still unknown. Across 41,603 production reconciliations over 90 days, nonzero $d$ spans about seven orders of magnitude, and no reliable empirical constant exists. We show that the count array of an IBLT has already measured $d$ before decoding. The measurement is in-band: it is carried by the recovery sketch itself and adds no bytes dedicated to estimation. A mapping-aware theorem extends the construction to Irregular, Rateless, and MET IBLTs. The protocol reads the estimate only after a decoding failure; we prove that the failure-conditioned lower quantile bounds the risk of underestimation, which gives the second-round capacity a configurable success-probability guarantee. The resulting self-sizing protocol attempts recovery with a small first-round sketch and stops on success; on failure it reads $d$, sizes the second round, and completes reconciliation in at most two rounds. Against a controlled oracle, communication is 1.29-1.47 times that of a scheme given $d$ in advance. Production workload characterization, relational-database replay, and a cross-city KV deployment confirm the end-to-end mechanism. In production on an Oracle-MySQL link, all completed runs succeeded within two rounds, over 90% on the 1-RTT fast path with a single 16 KB sketch.

==> figures/fig-protocol-sequence.tex <==
%
%
%
%
\providecommand{\ProtocolFigureXScale}{1}
\providecommand{\ProtocolFigureYScale}{1}
\providecommand{\ProtocolProtectionWidth}{132mm}
\providecommand{\ProtocolMeasureWidth}{72mm}
\begin{tikzpicture}[paper figure,
  xscale=\ProtocolFigureXScale,
  yscale=\ProtocolFigureYScale]
  %
  \node[paper endpoint, minimum width=19mm] (side-a) at (-6.15,0) {Side A};
  \node[paper endpoint, minimum width=19mm] (side-b) at ( 6.15,0)
    {Side B\\[-1pt]\footnotesize Controller};
  \draw[paper lifeline] (side-a.south) -- ++(0,-8.00);
  \draw[paper lifeline] (side-b.south) -- ++(0,-8.00);

  %
  \node[paper small text, text=PaperGray, anchor=east]
    at (-6.55,-1.05) {Round 1};
  \draw[paper flow]
    (-6.15,-1.35) --
    node[paper edge label] {IBLT, $M_1$ cells (fixed budget)}
    (6.15,-1.35);
  \node[paper annotation, anchor=north east, text width=55mm]
    (first-attempt) at (6.15,-1.72)
    {Save the pre-peeling counts; then attempt decoding.};

  %
  \node[paper small text, text=PaperGray, anchor=east]
    at (-6.55,-2.85) {success};
  \draw[paper return flow]
    (-6.15,-3.08) --
    node[paper edge label] {difference set; \texttt{DONE} (1 RTT)}
    (6.15,-3.08);

  %
  \draw[paper separator] (-6.72,-3.55) -- (6.72,-3.55);
  \node[paper small text, text=PaperGray, fill=white, inner xsep=2pt]
    at (0,-3.55) {on first-round failure};

  \node[paper mechanism, anchor=north, text width=\ProtocolMeasureWidth,
        font=\footnotesize]
    (measure) at (0,-3.88)
    {{\small\bfseries Measure and size the second round}\\[1pt]
     Estimate $\dhat$ from the saved counts; compute $M_2$.};

  %
  \node[paper small text, text=PaperGray, anchor=east]
    at (-6.55,-5.12) {Round 2};
  \draw[paper mechanism flow]
    (6.15,-5.55) --
    node[paper edge label, align=center]
      {read local fingerprint cache; \\ \texttt{REBUILD}$(M_2)$; fresh hash seed}
    (-6.15,-5.55);
  \draw[paper flow]
    (-6.15,-6.20) --
    node[paper edge label] {IBLT, $M_2$ cells}
    (6.15,-6.20);
  \node[paper annotation, anchor=north east, text width=49mm]
    (second-attempt) at (6.15,-6.55)
    {Jointly decode using the retained first-round residual core.};

  \draw[paper return flow]
    (-6.15,-8.12) --
    node[paper edge label] {difference set; \texttt{DONE} (2 RTT)}
    (6.15,-8.12);
\end{tikzpicture}

